Beyond Task Vectors: Selective Task Arithmetic Based on Importance Metrics

Pretrained models have revolutionized deep learning by enabling significant performance improvements across a wide range of tasks, leveraging large-scale, pre-learned knowledge representations. However, deploying these models in real-world multi-task learning (MTL) scenarios poses substantial challenges, primarily due to high computational costs and inefficiencies in inference. Traditional approaches such as pruning, quantization, and knowledge distillation have been explored to mitigate these issues, but they often fall short in fully addressing the complexities of multi-task environments. This paper introduces \textbf{\underline{S}}elective \textbf{\underline{T}}ask \textbf{\underline{A}}rithmetic \underline{\textbf{(STA)}}, a training-free framework designed to enhance multi-task performance through task-specific parameter fusion. STA addresses three key challenges: (i) \textbf{Parameter importance diversity: } Recognizing that different tasks relie on distinct parameters, STA employs a loss-sensitive parameter importance metric derived from a first-order Taylor expansion to accurately measure the importance of parameters for each task. (ii) \textbf{Over-reliance on hyperparameter tuning: }By enhancing the sparsity of task vectors through parameter importance metrics, STA reduces the need for extensive hyperparameter tuning, thereby improving the generalization and robustness of the model. (iii) \textbf{Neglect of other abilities in task arithmetic: } Previous works have largely overlooked the potential for more precise task forgetting. STA leverages its parameter importance metric to achieve more controlled and effective task forgetting, minimizing the impact of noisy elements that can degrade model performance. Experimental results demonstrate that STA achieves superior multi-task performance across benchmarks and excellent performance in task forgetting.

==> TaskVectorX/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, pre-trained models have become foundational to deep learning, enabling significant performance improvements across various tasks due to their capacity to utilize large-scale, pre-learned knowledge representations. Despite this success, deploying these models in real-world multi-task learning (MTL) \cite{chen2024multi} scenarios presents substantial challenges, particularly regarding computational cost and inference efficiency. This issue has spurred extensive research into model compression and optimization techniques, including pruning, quantization, and knowledge distillation. Among these, parameter-level task arithmetic \cite{ilharco2022editing} has emerged as a promising approach, allowing models to encapsulate essential knowledge without additional training. This method can reduce deployment costs by minimizing the parameter size while maintaining performance. However, effectively integrating task-specific parameters in a multi-task context remains challenging due to the inevitable noise introduced during the fusion process (a simple example is that if two parameters of different symbols are additionally fused, the result itself does not have a clear meaning).

%%% 放一张小图在第一页右上角，图去表述我们的任务场景是怎么样的（然后在引言合适的部分引用）
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\columnwidth]{./img/intro.pdf}
  \caption{Our STA method allows for more precise control of task vectors for better task arithmetic}
  \label{fig:intro}
  % \vspace{-20pt}
\end{figure}

Given shared pre-trained weights for different downstream models, the task arithmetic method calculates the \textbf{task vector} for each corresponding task by computing the difference between the fine-tuned weights and the pre-trained weights. This method multiplies the sum of these task vectors by a coefficient and adds them to the pre-trained weights to construct a model capable of performing multiple downstream tasks. Recently, several studies have proposed methods to enhance task arithmetic. For instance, \citet{yadav2024ties} improve fusion performance by removing smaller parameters and symbolic conflict parameters during the fusion of task vectors. \citet{yu2024language} utilize a random mask to ensure parameter sparsity, reducing noise during fusion. \citet{yang2023adamerging} optimize the coefficients of task vector fusion using test set data to enhance fusion performance. A recent work, PCB-Merging \cite{du2024parameter}, proposes making trade-offs in task fusion by measuring competition between parameters. However, the following issues are generally overlooked in these works:

\noindent 
%\underline{\textbf{(i)}} 
\textbf{Diversity in Parameter Importance:} Different tasks have unique dependencies on model parameters; parameters that are crucial for one task may be less significant or even irrelevant for another. Many existing methods overlook the potential improvements that accurate parameter importance measures can bring to task arithmetic, resulting in suboptimal performance.

\noindent 
%\underline{\textbf{(ii)}} 
\textbf{Over-reliance on hyperparameter tuning:} The aforementioned improvements based on task arithmetic still rely on coefficients in task vector fusion. Although these works have proposed methods for automatic optimization of these coefficients, concerns about generalization due to this dependency remain unresolved.

\noindent 
%\underline{\textbf{(iii)}} 
\textbf{Other abilities of task arithmetic are ignored:} While there are numerous studies based on task arithmetic mentioned above, to the best of our knowledge, only \citet{ilharco2022editing} consider task forgetting by directly subtracting a task-specific task vector from the parameters. However, some noisy elements can significantly impair the overall model function after the subtraction, leading to suboptimal results. This limitation greatly restricts the powerful potential of task arithmetic itself.

To address these challenges, we introduce \textbf{\underline{S}}elective \textbf{\underline{T}}ask \textbf{\underline{A}}rithmetic \underline{\textbf{(STA)}}, a novel training-free framework designed to enable efficient parameter fusion in multi-task learning. STA combines a loss-sensitive parameter importance metric(represents the degree to which a parameter contributes to a particular downstream task) derived from a first-order Taylor expansion with a gating mechanism for task-specific parameter selection (see \autoref{fig:intro}). Additionally, we applied this technique to the task forgetting scenario and obtained promising results. The main contributions of STA are: \textbf{\underline{(i)}} a loss-sensitive metric based on first-order Taylor expansion, which provides a precise and computationally efficient assessment of parameter importance for each task; \textbf{\underline{(ii)}} leveraging precise parameter importance measurement, STA can accurately sparsify the task vector of each downstream task model, making it fully suitable for arbitrary task arithmetic operations. This high sparsity also eliminates dependency on the choice of coefficients when performing task arithmetic operations; and \textbf{\underline{(iii)}} our STA method surpasses the current state-of-the-art in different arithmetic tasks, including task fusion and task forgetting.

%% 可以放框架图
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{./img/overview-deep.pdf}
  % \vspace{-5pt}
  \caption{The overview of our proposed Selective Task Arithmetic. In STA, we measure the importance of the task vector through the loss-sensitive parameter importance measurement method, and then complete the sparsification of the task vector through the importance to obtain the sparse task vector, and then use this task vector to complete tasks such as task fusion or specific task forgetting. A more detailed description of the process is provided in \autoref{sec:method}.}
  \label{fig:overview}
  % \vspace{-10pt}
\end{figure*}

==> TaskVectorX/sec/2_related.tex <==
\section{Related Work}
\label{sec:related}


